Normal Forms of second order Ordinary Differential Equations $y_{xx}=J(x,y,y_{x})$ under Fibre-Preserving Maps

We study the equivalence problem of classifying second order ordinary differential equations $y_{xx}=J(x,y,y_{x})$ modulo fibre-preserving point transformations $x\longmapsto \varphi(x)$, $y\longmapsto \psi(x,y)$ by using Moser's method of normal forms. We first compute a basis of the Lie algebra ${\frak{g}}_{{\{y_{xx}=0\}}}$ of fibre-preserving symmetries of $y_{xx}=0$. In the formal theory of Moser's method, this Lie algebra is used to give an explicit description of the set of normal forms $\mathcal{N}$, and we show that the set is an ideal in the space of formal power series. We then show the existence of the normal forms by studying flows of suitable vector fields with appropriate corrections by the Cauchy-Kovalevskaya theorem. As an application, we show how normal forms can be used to prove that the identical vanishing of Hsu-Kamran primary invariants directly imply that the second order differential equation is fibre-preserving point equivalent to $y_{xx}=0$.

==> bibliography <==
\begin{thebibliography}{225}

{\bf\bibitem{Beloshapka-Ezhov-Schmalz-2007}
{\sc Beloshapka}}, V.K., {\sc Ezhov}, V., {\sc Schmalz}, G.: {\em Canonical Cartan connection and holomorphic invariants
on Engel CR manifolds}. Russ. J. Math. Phys. 14(2), 121–133 (2007)

{\bf\bibitem{Bluman-Kumei-1989}
{\sc Bluman}}, G.W.; {\sc Kumei}, S.:
{\em Symmetries and differential equations}, 
Springer-Verlag, Berlin, 1989, xiv+412~pp.

\smallskip

{\bf\bibitem{BCGGG-1991}
 {\sc Bryant}}, R. L.; {\sc Chern}, S. S.; {\sc Gardner}, R. B.; {\sc Goldschmidt}, H. L.; {\sc Griffiths}, P. A.: {\em Exterior differential systems.} Mathematical Sciences Research Institute Publications, 18. Springer-Verlag, New York, 1991. viii+475 pp. ISBN: 0-387-97411-3

\smallskip

{\bf\bibitem{Bryant-1982}
{\sc Bryant}}, Robert L.: {\em Holomorphic curves in Lorentzian CR-manifolds}. Trans. Amer. Math. Soc. 272 (1982), no. 1, 203–221.

\smallskip

{\bf\bibitem{Cartan-1}
{\sc Cartan}}, \'{E}.: {\em Sur la g\'{e}om\'{e}trie pseudo-conforme des hypersurfaces de l’espace de deux variables com-
plexes, I}. Ann. Math. Pura Appl. 11, 17–90 (1932)

\smallskip

{\bf\bibitem{Cartan-2}
{\sc Cartan}}, \'{E}.: {\em Sur la g\'{e}om\'{e}trie pseudo-conforme des hypersurfaces de l’espace de deux variables com-
plexes, II}. Ann. Scuola Norm. Sup. Pisa 1, 333–354 (1932

{\bf\bibitem{Chen-Shaw}
{\sc Chen}}, So-Chin; {\sc Shaw}, Mei-Chi: {\em Partial differential equations in several complex variables. AMS/IP Studies in Advanced Mathematics}, 19. American Mathematical Society, Providence, RI; International Press, Boston, MA, 2001. xii+380 pp. ISBN: 0-8218-1062-6 

\smallskip
{\bf\bibitem{Chern-Moser-1974}
 {\sc Chern}}, S. S.; {\sc Moser}, J. K.: {\em Real hypersurfaces in complex manifolds}. Acta Math. 133 (1974), 219–271. 
 
 \smallskip

{\bf\bibitem{Ezhov-Isaev-Schmalz-1999}
{\sc Ezhov}}, V.; {\sc Isaev}, A.V.; {\sc Schmalz},G.: {\em Invariants of elliptic and hyperbolic CR-structures of codimension
2}. Int. J. Math. 10(1), 1–52 (1999)

\smallskip

{\bf\bibitem{Ezhov-McLaughlin-Schmalz-2011}
{\sc Ezhov}}, V., {\sc McLaughlin}, B., {\sc Schmalz}, G.: {\em From Cartan to Tanaka: getting real in the complex world}.
Not. Am. Math. Soc. 58(1), 20–27 (2011)

\smallskip

{\bf\bibitem{Isaev-Zaitsev-2013}
{\sc Isaev}}, A., {\sc Zaitsev}, D.: {\em Reduction of five-dimensional uniformly Levi degenerate CR structures to
absolute parallelisms}. J. Geom. Anal. 23(3), 1571–1605 (2013)


\smallskip

{\bf\bibitem{Cartanforbeginners}
 {\sc Ivey}}, Thomas A.; {\sc Landsberg}, Joseph M. {\em Cartan for beginners.: Differential geometry via moving frames and exterior differential systems}. Second edition [of MR2003610]. Graduate Studies in Mathematics, 175. American Mathematical Society, Providence, RI, 2016. xviii + 453 pp. ISBN: 978-1-4704-0986-9

\smallskip

{\bf\bibitem{Medori-Spiro-2014}
{\sc Medori}}, C.; {\sc Spiro}, A.: {\em The equivalence problem for five-dimensional Levi degenerate CR manifolds}.
Int. Math. Res. Not. IMRN 20, 5602–5647 (2014)

\smallskip

{\bf\bibitem{Merker-2008}
{\sc Merker}}, J.:
{\em Lie symmetries and CR geometry}, J.
Mathematical Sciences, {\bf 154} (2008), no.~6, 817--922.

\smallskip

{\bf\bibitem{Merker-Manuscript-2013-1}
{\sc Merker}}, J.: {\em Equivalences of 5-dimensional CRmanifolds,III: Six models and (very) elementary normalizations}. arXiv:1311.7522

\smallskip

{\bf\bibitem{Merker-Manuscript-2013-2}
{\sc Merker}}, J.: {\em Equivalences of 5-dimensional CR manifolds, IV: Six ambiguity matrix groups (Initial G-structures)}. arXiv:1312.1084

\smallskip

{\bf\bibitem{Merker-Manuscript-2013-3}
{\sc Merker}}, J.: {\em Equivalences of 5-dimensional CR-manifolds V: Six initial frames and coframes; Explicitness obstacles}. arXiv:1312.5688

\smallskip

{\bf\bibitem{Merker-Lie-2015} 
{\sc Merker}},~J. (Editor); {\sc Lie},~S. (Author):
{\em Theory of Transformation Groups I. 
General Properties of Continuous Transformation Groups. 
A Contemporary Approach and Translation}, 
Springer-Verlag, Berlin, Heidelberg, 2015, xv+643~pp.

\smallskip

{\bf\bibitem{Merker-Manuscript-Lorentzian} 
{\sc Merker}},~J.:
{\em Holomorphic Curves in Lorentzian CR
Manifolds:
Effective aspects },
written manuscript.

\smallskip

{\bf\bibitem{Merker-Pocchiola-2018}
{\sc Merker}}, J.; {\sc Pocchiola} S.
{\em Explicit Absolute Parallelism for 2-Nondegenerate Real Hypersurfaces $M^5 \subset \mathbb {C}^3$ of Constant Levi Rank 1}. The Journal of Geometric Analysis (Feb 2018), pp~1-42.

\smallskip

{\bf\bibitem{Olver-1995} 
{\sc Olver}},~P.J.:
{\em Equivalence, Invariance and Symmetries}. Cambridge, Cambridge
University Press, 1995, xvi+525~pp.

\smallskip

{\bf\bibitem{Pocchiola-Manuscript-2014-1}
{\sc Pocchiola}}, S.: {\em Canonical Cartan connection for 4-dimensional CR-manifolds belonging to general
class II}. arXiv:1405.1341

\smallskip


{\bf\bibitem{Pocchiola-Manuscript-2014-2}
{\sc Pocchiola}}, S.: {\em Canonical Cartan connection for 5-dimensional CR-manifolds belonging to general
class III2}. arXiv:1405.1342


\smallskip

{\bf\bibitem{Sabzevari-Merker-2014}
{\sc Sabzevari}}, M.; {\sc Merker}, J.: {\em The Cartan equivalence problem for Levi-non-degenerate real hypersurfaces $M^{3}\subset \mathbb{C}^{2}$}. Izvestiya Math. 78, 1158–1194 (2014)

\smallskip

{\bf\bibitem{Sabzevari-Merker-Manuscript-2014}
{\sc Sabzevari}}, M.; {\sc Merker}, J.: {\em Cartan equivalences for 5-dimensional CR-manifolds in $\mathbb{C}^{4}$}. arXiv:1401.4297

\smallskip

{\bf\bibitem{Schmalz-Spiro-2006}
{\sc Schmalz}}, G.; {\sc Spiro}, A.: {\em Explicit construction of a Chern-Moser connection for CR manifolds of codimension two}. Ann. Mat. Pura Appl. 4 185(3), 337–379 (2006)

\smallskip


{\bf\bibitem{Sommer-1959} 
{\sc Sommer}},~F.:
{\em Komplexe-analytische Bl\"atterung reeller Hyperfl\"achen im }$\mathbb{C}^{n}$,
 Math. Ann. {\bf{137}} (1959), S392-411.
 
 {\bf\bibitem{Shabat-1992}
 {\sc Shabat}}, B.V.:
 {\em Introduction to Complex Analysis. Part II: Several Complex
 Variables.} Translations of Mathematical Monographs, 
 Amer. Math. Soc., vol. 110, 1992, x+371~pp.
 
 \smallskip
 
 {\bf\bibitem{Tanaka}
{\sc Tanaka}}, N.: {\em On the pseudo-conformal geometry of hypersurfaces of the space of n complex variables}.
J. Math. Soc. Jpn. 14, 397–429 (1962)
 
\end{thebibliography}



==> introduction.tex <==
% !TEX root = NAME.tex

\section{Introduction}


==> title-author <==
$\:$

\bigskip\bigskip\bigskip\bigskip\bigskip

\begin{center}

{\large\bf
The Geometry of Chern-Moser normal forms in dimensional 2
}
\label{immersion-bidisk}

\bigskip\bigskip

Zhangchi {\sc Chen},\quad Wei Guo {\sc Foo},\quad Jo\"{e}l {\sc Merker},\quad The-Anh {\sc Ta}

\smallskip

%{\large\footnotesize\sf D\'epartement de Math\'ematiques d'Orsay}

%{\large\footnotesize\sf Université Paris-Sud, France}

\end{center}\bigskip

\bigskip


==> write.tex <==

%%% PARIS %%%

\setlength{\textheight}{12.05cm}
\setlength{\textwidth}{14.05cm}
\voffset -4.05cm
\hoffset -4.25cm

%%% AVANNE %%%

%\setlength{\textheight}{13.5cm}
%\voffset -3.85cm
%\hoffset -4.25cm


